A Modular Platform For Collaborative, Distributed Sensor Fusion

Leading autonomous vehicle (AV) platforms and testing infrastructures are, unfortunately, proprietary and closed-source. Thus, it is difficult to evaluate how well safety-critical AVs perform and how safe they truly are. Similarly, few platforms exist for much-needed multi-agent analysis. To provide a starting point for analysis of sensor fusion and collaborative & distributed sensing, we design an accessible, modular sensing platform with AVstack. We build collaborative and distributed camera-radar fusion algorithms and demonstrate an evaluation ecosystem of AV datasets, physics-based simulators, and hardware in the physical world. This three-part ecosystem enables testing next-generation configurations that are prohibitively challenging in existing development platforms.

==> tables/table_metrics.tex <==
% ===========
\begin{table}[t!]
    \centering
    \begin{tabular}{||l l||}
        \hline
        \textbf{Module} & \textbf{Metric} \\
        \hline
        Perception & \tworowsubtableleft{False Positive Rate (FPR), Precision, mAP}{False Negative Rate (FNR), Recall, IoU}\\
        \hline
        Tracking   & \tworowsubtableleft{\tworowsubtableleft{IoU, False Track Rate (FTR)}{Missed Track Rate (MTR)~\cite{2008trackingeval}}}{\tworowsubtableleft{Higher Order Tracking Accuracy (HOTA)~\cite{2021hotametric}}{CLEAR~\cite{2008CLEARmetrics}, VACE~\cite{2017VACEmetrics}, IDEucl~\cite{2021hotametric}}} \\
        \hline
        Prediction & \tworowsubtableleft{Average Displacement Error (ADE)~\cite{2009ADEmetric}}{Final Displacement Error (FDE)~\cite{2016sociallstm}}\\
        \hline
        Planning   & \tworowsubtableleft{Responsibility Sensitive Safety (RSS)~\cite{2017rsssafety}}{Path KL Divergence~\cite{2020nuscenesdataset}}\\
        \hline
        Control    & \tworowsubtableleft{Responsibility Sensitive Safety (RSS)~\cite{2017rsssafety}}{CARLA Leaderboard Benchmark~\cite{2017carla}}\\
        \hline
    \end{tabular}
    \caption{\texttt{AVstack} unifies metrics for longitudinal testing while previous works only tested isolated components. \texttt{AVstack} uniquely incorporates the RSS safety metric.}
    \vspace{-20pt}
    \label{tab:metrics}
\end{table}
% ===========
